Trust-aware Control for Intelligent Transportation Systems

Many intelligent transportation systems are multi-agent systems, i.e., both the traffic participants and the subsystems within the transportation infrastructure can be modeled as interacting agents. The use of AI-based methods to achieve coordination among the different agents systems can provide greater safety over transportation systems containing only human-operated vehicles, and also improve the system efficiency in terms of traffic throughput, sensing range, and enabling collaborative tasks. However, increased autonomy makes the transportation infrastructure vulnerable to compromised vehicular agents or infrastructure. This paper proposes a new framework by embedding the trust authority into transportation infrastructure to systematically quantify the trustworthiness of agents using an epistemic logic known as subjective logic. In this paper, we make the following novel contributions: (i) We propose a framework for using the quantified trustworthiness of agents to enable trust-aware coordination and control. (ii) We demonstrate how to synthesize trust-aware controllers using an approach based on reinforcement learning. (iii) We comprehensively analyze an autonomous intersection management (AIM) case study and develop a trust-aware version called AIM-Trust that leads to lower accident rates in scenarios consisting of a mixture of trusted and untrusted agents.

==> sections/intro.tex <==
Multi-agent autonomous cyber-physical systems (MACPSs) are rapidly becoming pervasive in the automotive, avionic, and robotic domains. For example, in the automotive domain, many functionalities such as autonomous intersection 
management \cite{dresner2004multiagent,sharon2017protocol}, cooperative adaptive platoons \cite{milanes2013cooperative}, 
cooperative highway merging \cite{rios2016automated, ntousakis2016optimal}, and cooperative collision avoidance 
\cite{alonso2018cooperative,bin2017research} can be modeled as MACPSs. With increasing adoption of unmanned aerial vehicles (UAVs) in the national airspace \cite{sharma2020communication} and ground robots such as intelligent firefighting robots \cite{rakib2016design} in disaster management situations, we can envision 
a future life with MACPSs. There has been significant emphasis on reasoning about the security and privacy of CPS applications \cite{khalid2018security, sun2016cyber,alguliyev2018cyber,habibzadeh2019survey,gupta2020smart,giraldo2017security}, using ideas from control theory and cyber-security. However, the notion of 
trustworthiness has received limited attention. 

What makes a CPS agent trustworthy? While this is a nuanced question, we propose a mathematically precise definition for trustworthiness that relies on two key principles: (\textit{i}) trusted or reliable agents obey the control actions suggested
by a central (or distributed) coordinator, (\textit{ii}) trusted agents do not provide false information. We assume that a {\em trust authority} (TA) can evaluate the trustworthiness of an agent through two kinds of observations: direct
observation of the agent's behavior and indirect information / observation gleaned from local trust authorities. Each of these observations represent evidence that enhances the TA's belief or disbelief in the agent (depending on
whether the evidence respectively indicates a desired or undesired behavior 
of the agent). For agents that the TA has no opportunity to observe, the TA has
no belief or disbelief in the agent, but instead has uncertainty about its 
trustworthiness. These ideas are rigorously developed in an {\em epistemic} 
logic called {\em subjective logic} that we employ for trust quantification.

We provide a conceptual depiction of a trust-aware MACPS in Fig.\ref{fig:CPS}. 
The system consists of a number of distributed agents, each with their own 
sensors, actuators and local control algorithms. The coordination and 
cooperation among the agents is achieved through either a centralized or 
a distributed control algorithm. Traditionally, the only input to such a 
controller is the global specification of desired behavior (encoding both
mission objectives for the MACPS and safety constraints). In our framework,
we additionally provide a trustworthiness score for all agents. This score
is computed by a TA from observations of agents (reported
through the agents' sensing and communication modules). The TA may also 
get information from local trust authorities (LTAs) that themselves may or 
may not be trusted. The TA may store the trustworthiness scores
for agents in a cloud-based infrastructure. The trust-aware control 
algorithm uses the global specification and trustworthiness scores to 
give control actions to the agents in the MACPS, which the agents can
choose to act on through their decision-making, planning and actuation modules. 

% The blue shaded area contains embedded control and sensing 
% technologies to monitor and control physical systems 
% \cite{derler2011modeling}. 


% In multi-agent systems, embedded devices and agents may operate as part of sources of uncertainty and lack security features \cite{ammar2020simple}. 
% Such uncertainty and untrusted entities in systems effect control outcomes in multiple ways. 
% Hence, in this work, we bring the trustworthiness of agents in multi-agent CPSs and envision a cloud-based (or edge-based) architecture where trustworthiness of agents are stored and accessible to authenticated control algorithms as shown in Fig. \ref{fig:CPS}. 
% Through trust authorities, quantitative trustworthiness scores of agents are evaluated and utilized in trust-aware control technologies to coordinate within scenarios where there exist untrustworthy agents. 
% Controllers in such systems receive inputs to a system, which include the environment assumptions, and compute the output guarantees satisfying specific properties. 

\begin{figure}
    \centering
    \includegraphics[width=.9\columnwidth]{fig/CPS-Trust-2.png}
    \caption{A trust-aware cyber-physical system.}
    \label{fig:CPS}
\end{figure}

In light of the above-mentioned challenges, we provide a comprehensive trust quantification analysis and trust-aware control algorithms for an autonomous
intersection management (AIM) system. The AIM is a visionary system 
proposed by Dresner and Stone \cite{dresner2008multiagent}  to reduce the 
increasing traffic load of current transportation infrastructure and the 
resulting transportation delays \cite{hausknecht2011autonomous}. It
promises %autonomous 
to improve the intersection efficiency under the 
assumption that all vehicles communicate with the AIM and strictly follow
the instructions.  Compared to conventional intersection control 
mechanisms such as stop signs and traffic signals, AIM policies provide
consistently high traffic throughput while ensuring safety of the traffic
participants \cite{hausknecht2011autonomous}. 

In real-world scenarios, driving is fraught with uncertainties arising
from fallible as well as compromised human drivers, defective sensors 
or actuators, noisy sensing environments, and V2X communication. While existing work on AIM focuses on extending to scenarios with human-driven or semi-autonomous vehicles \cite{sharon2017protocol,au2015autonomous}, it does not 
account for the possibility of such systemic or adversarial 
uncertainties. Thus, untrustworthiness arising out of uncertainty
can invalidate the benefits of AIM. A key contribution in this paper
is to showcase AIM as a detailed case study to highlight our algorithms 
for trust quantification and trust-aware control for MACPS. We show how we can
modify AIM to obtain AIM-Trust that uses trustworthiness scores of 
traffic participants to generate trust-aware control actions. We 
use the reinforcement learning (RL) framework, where the action
space for the RL problem is the allocation of space-time buffers 
for cars to navigate the intersection modulated by their 
trustworthiness, and the reward space is defined in terms of collision
freedom and intersection throughput. Our formulation allows AIM-Trust
to explore a trade-off between performance (throughput) and safety
(collision freedom). To summarize, the main contributions of this
paper are as follows:
\begin{itemize}[leftmargin=*]
    \item We propose a method to quantify trustworthiness scores for individual agents in a MACPS.
    \item We provide a general and abstract framework for incorporating trust in generating control actions that guarantee the satisfaction
    of a global MACPS specification.
    \item We showcase our trust quantification and trust-aware control
    methodology through a detailed case study of Autonomous Intersection 
    Management (AIM).
    \item We demonstrate how to embed the trustworthiness scores in a RL-based policy synthesis procedure. 
    \item Our empirical results show higher safety (at least $18.18\%$ and up to $89.28\%$ collision reduction) and efficiency ($15.53\%$ throughput improvement on average) of intersection management under the AIM-Trust controller compared to classical AIM that does not account for trustworthiness of vehicles.
\end{itemize}

% we focus on intelligent transportation multi-agent cyber-physical
% systems and demonstrate trustworthiness quantification and control methods with
% autonomous intersection management applications. 
% Self-driving cars along with intelligent transportation systems have become a rapidly approaching future where the autonomous vehicles work hand in hand with traffic control mechanisms, such as intelligent intersection managing mechanisms.
% Intersections and intersection control mechanisms, such as traffic lights and stop signs, contribute to higher rates of accidents and traffic flow bottlenecks \cite{bashiri2018paim,chang2003relationship,choi2010crash}. 

% Since untrustworthy human drivers and adversarial autonomous vehicles would not follow the instructions strictly and they are not $100\%$ trustworthy, they may or may not follow the IM's simulated trajectories within the range of error tolerance. Therefore, AIM does not outperform conventional traffic control mechanisms in terms of traffic throughput and/or collision rate or even is not applicable in such cases. 

